Reinforcement Learning with LTL and $\omega$-Regular Objectives via Optimality-Preserving Translation to Average Rewards

Linear temporal logic (LTL) and, more generally, $\omega$-regular objectives are alternatives to the traditional discount sum and average reward objectives in reinforcement learning (RL), offering the advantage of greater comprehensibility and hence explainability. In this work, we study the relationship between these objectives. Our main result is that each RL problem for $\omega$-regular objectives can be reduced to a limit-average reward problem in an optimality-preserving fashion, via (finite-memory) reward machines. Furthermore, we demonstrate the efficacy of this approach by showing that optimal policies for limit-average problems can be found asymptotically by solving a sequence of discount-sum problems approximately. Consequently, we resolve an open problem: optimal policies for LTL and $\omega$-regular objectives can be learned asymptotically.

==> learning.tex <==
\newcommand{\simu}{\mathcal{X}}
\newcommand{\mchain}{M}
\newcommand{\tmix}{T_{\textrm{mix}}}
\newcommand{\ecom}{\mathcal{C}}
\newcommand{\reachcom}{x}
\newcommand{\rewardcom}{y}
\newcommand{\remove}[1]{}

Having already established the constructs from $\omega$-regular languages to average reward machines, we now aim to devise a reinforcement learning algorithm for the latter. A negative result from~\cite{Alur:2022} indicates that such an algorithm cannot be PAC-MDP. Therefore, the most desirable outcome would be an algorithm that converge in the limit. We make the following assumptions:

\noindent{\bf Assumption 1}. The readers are familiar with the following terminologies about Markov chains~(e.g.~\cite{Puterman:1994,Sutton:2018}) such as irreducible chain, aperiodic chain, total invariance measure, unichain, multichain, stationary distribution, limiting distribution.   A Markov chain is \emph{ergodic} if it is irreducible and aperiodic. We let $\mdp_{\pi}$ denote the induced MDP of $\mdp$ w.r.t. the policy $\pi$.

\noindent {\bf Assumption 2}.~The scalar rewards are normalized in the range $[0,1]$. The MDP is finite and every state has at least one transition.  This ensures the existence of at least one transition with a non-zero probability and at least one irreducible chain under any memoryless deterministic policy. In relation to each MDP $\mdp$, we are provided with a simulator $\simu^\mdp: S \times A \rightarrow \mathcal{D}(S)$, where $\simu(s,a) = s'$ with a probability of $P(s,a,s')$.



\ar{Remove 3 from the formal assumption}

 The following well-known result enables us to narrow down our search for the optimal solution to the finite set of deterministic memoryless policies:
\begin{proposition}[{\cite[p.451]{Puterman:1994}}]\label{prop:opt-avg-pol}
	There exists an optimal deterministic memoryless policy for average reward function.
\end{proposition}


Hereafter, unless stated otherwise, every policy is assumed to be deterministic memoryless. 

 Let $\mdp = (S,A,s_0,P)$ be an MDP and $\rfun = (U,u_0,\delta_u,\delta_r)$ a reward machine. Their product is the MDP $\mdp' = \mdp \ltimes \rfun = (S',A,s'_0,P')$ where $S' = S \times A$, $s'_0 = (s_0,u_0)$, $P'((s,u),a,(s',u')) = \mathds{1}{\left(u'=\delta_u(s,a,s')\right)} \cdot P(s,a,s')$. The induced reward function $\rfun'$ of $\mdp'$ satisfies $\rfun'((s,u),a,(s',u'))=\delta_r(u,(s,a,s'))$. 
 
For an MDP $\mdp$ and policy $\pi$, we let $\mathsf{EC}(\mdp,\pi)= \{\ecom_1,\ldots,\ecom_n\}$ where $n \geq 1$ denote the set of ECs in the induced MDP $\mdp_\pi$. It can be checked that $\ecom_1,\ldots,\ecom_n$ are simple and pair-wise disjoint as each of them corresponds to an irreducible Markov chain. Also, we let $\reachcom^\mdp_\pi(\ecom_i)$ and $\rewardcom^\mdp_\pi(\ecom_i,\rfun)$ denote the reachability probability  and the limit-average reward of $\ecom_i$\footnote{Since $\ecom_i$ is unchain, its limit-average reward is uniquely determined regardless of the initial distribution.}  in $\mdp_\pi$, respectively: 
\[
\reachcom^\mdp_\pi(\ecom_i) ~\defi~ \Pr_{\zeta \in \mathcal{D}^\mdp_\pi}\left[ \textrm{$\zeta$ reaches $\ecom_i$} \right] \hspace{2em}\textrm{and}\hspace{2em} \rewardcom^\mdp_\pi(\ecom_i,\rfun)~\defi~ \lim_{t \rightarrow \infty} \mathbb{E}_{\zeta \in \mathcal{D}^\mdp_\pi}\left[ \vfuns_{\rfun^{\textrm{avg}}}^t(\zeta)~|~ \textrm{$\zeta$ reaches $\ecom_i$}\right]
\]

 The following result indicates that the limit-average reward for a policy can be determined by considering the reachability probabilities and limit-average rewards of the SECs in the induced MDP:
\begin{proposition}\label{prop:avg-policy}
	Let $\pi$ be a policy of the MDP $\mdp$ with the reward function $\rfun$.  Then $\vfuns^{\mdp}_{\rfun^{\textrm{avg}}}(\pi) ~=~ \sum_{\ecom \in \mathsf{EC}(\mdp,\pi)} \reachcom^\mdp_\pi(\ecom) \cdot \rewardcom^\mdp_\pi(\ecom,\rfun)$.
\end{proposition}
\begin{proof}
 Note that $\ecom_1,\ldots,\ecom_n$ are simple and pair-wise disjoint. By~\cref{prop:end-components} and~\cref{prop:asec}:
	\[
	\begin{array}{lll}
		\vfuns^{\mdp}_{\rfun^{\textrm{avg}}}(\pi) &=& \lim_{t \rightarrow \infty}{\sum_{i=1}^{n}\mathbb{E}_{\run \in \mathcal{D}^\mdp_\pi}\left[ \vfuns^t_{\rfun^{\textrm{avg}}}(\run)~|~ \textrm{$\run$ reaches $\ecom_i$}\right]}
		\\
		&=& \sum_{i=1}^{n}\Pr_{\run \in \mathcal{D}^\mdp_\pi}\left[\textrm{$\run$ reaches $\ecom_i$}\right] \cdot \lim_{t \rightarrow \infty} \mathbb{E}_{\zeta \in \mathcal{D}^\mdp_\pi}\left[ \vfuns_{\rfun^{\textrm{avg}}}^t(\zeta)~|~ \textrm{$\zeta$ reaches $\ecom_i$}\right]
		\\
		 &=& \sum_{i=1}^{n} \sum_{i=1}^{n} \reachcom^\mdp_\pi(\ecom_i) \cdot \rewardcom^\mdp_\pi(\ecom_i,\rfun).
	\end{array}
	\]

Hence, we are done.
\end{proof}


For the rest of this section, we will establish the following result: the existence of an $\omega$-PAC RL algorithm  for the general $\mdp$ w.r.t. the average reward machine $\rfun$. This results holds true under the condition that we also possess a positive lower bound $0 < \beta < \min{\{p^{\mdp}_{\min},1/T_{\textrm{mix}}^{\mdp \ltimes \rfun}\}}$. Here, $p_{\min}^{\mdp}$ represents the lowest non-zero transition probability in  $\mdp$, and $T_{\textrm{mix}}^{\mdp \ltimes \rfun}$ denotes the \emph{adjusted mixing time} (\cref{def:mixing}) of the product MDP $\mdp \ltimes \rfun$:

\begin{theorem}\label{thm:learning-optimal}
	There is an algorithm $\omega$-PAC which input (1) a simulator for the MDP $\mdp$, (2) a reward machine $\rfun$, (3) a positive lower bound  $0 < \beta \leq \min{\{p^{\mdp}_{\min},1/T_{\textrm{mix}}^{\mdp \ltimes \rfun}\}}$ , (4)~$\epsilon,\delta > 0$ and $\epsilon < 2$, and outputs a policy $\pi$ such that 
	\[
	\Pr[\vfun{\mdp}{\rfun}(\pi) ~\geq~ \vfuns^*(\mdp,\rfun) - \delta] ~\geq~ 1 - \epsilon.
	\]
\end{theorem}
\remove{
The following well-known result allows us to restrict our search of optimal solution to the finite set of deterministic memoryless policies:
\begin{proposition}[{\cite[p.326]{Puterman:1994}}]\label{prop:opt-avg-pol}
	There exists an optimal deterministic memoryless policy for average reward function.
\end{proposition}

Hereafter, unless stated otherwise, every policy is assumed to be deterministic memoryless. The following result tells us how to compute the limit-average reward for a policy:
\begin{proposition}\label{prop:avg-policy}
	Let $\pi$ be a policy of the MDP $\mdp$ with the reward function $\rfun$.  Suppose $\{\ecom_1,\ldots,\ecom_n\}$ is the set of ECs in the induced MDP $\mdp_\pi$. Then:
	\begin{enumerate}
		\item $\ecom_1,\ldots,\ecom_n$ are simple and pair-wise disjoint.
		\item Let $x_i$ and $y_i$ be the reachbility probability and  the limit-average reward of $\ecom_i$, respectively. Then $\vfuns^{\mdp}_{\rfun^{\textrm{avg}}}(\pi) = \sum_{i=1}^{n} x_i \cdot y_i$.
	\end{enumerate}
\end{proposition}
\begin{proof}
	For (1), $\ecom_i$ is simple because $\pi$ is deterministic. Now, suppose $\ecom_i$ and $\ecom_j$ share a common state $s$.  Then their union is an EC which is an SEC by (1). This is, however, impossible unless $i = j$.
	
	For (2), note that each $\ecom_i$ is a unichain and thus its limit-average reward is uniquely determined regardless of the initial state. Thus the term $y_i$ is well-defined. By~\cref{lem:ec}, we have:
	\[
	\begin{array}{lll}
		\vfuns^{\mdp}_{\rfun^{\textrm{avg}}}(\pi) &=& \lim_{t \rightarrow \infty}{\sum_{i=1}^{n}\mathbb{E}_{\run \in \mathcal{D}^\mdp_\pi}\left[ \vfuns^t_{\rfun^{\textrm{avg}}}(\run)~|~ \textrm{$\run$ enters $\ecom_i$}\right]}
		\\
		&=& \sum_{i=1}^{n}\underbrace{\Pr_{\run \in \mathcal{D}^\mdp_\pi}\left[\textrm{$\run$ enters $\ecom_i$}\right]}_{x_i} \cdot \underbrace{\lim_{t \rightarrow \infty} \vfuns^t_{\rfun^{\textrm{avg}}}(\run~|~\textrm{$\run$ enters $\ecom_i$})}_{y_i} ~=~ \sum_{i=1}^{n} x_i \cdot y_i.
	\end{array}
	\]
\end{proof}
}
At the high-level viewpoint, our approach is simple. First, we sample each state-action pair in $\mdp$ to obtain a good approximation $\overline{\mdp}$. We then compute the exact optimal deterministic memoryless policy of $\overline{\mdp} \ltimes \rfun$ and transform it into a deterministic finite-memory policy for $\mdp$. Knowing the positive lower bound $\beta$ allows us to sample $\overline{\mdp}$ with arbitrary low error and high confidence, ensuring that the optimal policy of $\overline{\mdp}$ is also very close to optimal w.r.t. $\mdp$. Intuitively, $p_{\min}^{\mdp}$ tells us the convergence rate for a run of a (deterministic memoryless) policy to enter a simple EC whereas $1/T_{\textrm{mix}}^{\mdp \ltimes \rfun}$ tells us the convergence rate of a run, once entered a simple EC, converging to the limit-average reward of that EC.

\begin{definition}
	Given an MDP $\mdp = (S,A,s_0,P)$. The estimate of $\mdp$ is an MDP $\overline{\mdp} = (S,A,s_0,\overline{P})$ where $\overline{P}$ is obtained by sampling the action-state pairs in $\mdp$ (e.g. by maintaining a frequency count $F: S \times A \times S \rightarrow \mathbb{N}$ to compute $\overline{P}$). Let $\delta > 0$. We say $\overline{\mdp}$ is $(\mdp,\delta)$-estimate if  for every transition $(s,a,s') \in S \times A \times S$, $|\overline{P}(s,a,s') - P(s,a,s')| < \delta$ and $\overline{P}(s,a,s') > 0$ iff $P(s,a,s') > 0$, i.e. they have the same structure.
\end{definition}
\remove{
\begin{proposition}\label{prop:estimate-mdp}
		Let $\overline{\mdp}$ be $(\mdp,\delta)$-estimate where $\delta < p_{\min}^{\mdp}$. Then  $\overline{\mdp}$ and $\mdp$ have the same structure, i.e. $\overline{P}(s,a,s') > 0$ iff $P(s,a,s') > 0$ for every  transition $(s,a,s')$.
\end{proposition}
\begin{proof}
	 We show that the following two cases are impossible:
	\begin{enumerate}
		\item $P(s,a,s') = 0$ and $\overline{P}(s,a,s') > 0$. This cannot happen as the simulator is accurate.
		\item $P(s,a,s') > 0$ and $\overline{P}(s,a,s') = 0$. Then $p_{\min}^{\mdp} \leq |P(s,a,s') - \overline{P}(s,a,s')| \leq \delta$ which is a contradiction.
	\end{enumerate}
	Hence, $\overline{\mdp}$ and $\mdp$ have the same structure.
\end{proof}
}
\begin{definition}\label{def:mixing} 	Given an MDP $\mdp$. Let $\mathsf{SEC}(\mdp) = \{\ecom_1,\ldots,\ecom_n\}$ where $n \geq 1$ be the set of SECs in $\mdp$. Each $\ecom$ induces an irreducible Markov chain represented by a transition matrix $\mchain$. We can make $\mchain$  ergodic using the transformation $\hat{\mchain}~\defi~\frac{1}{2}(\mchain + I)$. It is well-known that the unique stationary distribution of an ergodic chain is also the limiting distribution~CITE. The distance to $\pi$ w.r.t. $\hat{\mchain}$ is defined as:
	\[
	d^{\hat{\mchain}}(t)~\defi~\max_x{\norm{\hat{\mchain}^t(x,\cdot) - \pi}_{\textrm{TV}}}
	\]
	where $\hat{\mchain}^t(x,\cdot)$ is the distribution of states that are reachable from $x$ after $t$ steps and $\norm{\cdot}_{\textrm{TV}}$ is the total variation measure. 
	
	Let $\epsilon > 0$. The \emph{ergodic $\epsilon$-mixing time} of $\ecom$ and $\mdp$ are defined as:
	\[
	\tmix^{\ecom}(\epsilon)=\tmix^{\hat{\mchain}}(\epsilon) ~\defi~ \min{\{t:d^{\hat{\mchain}}(t) \leq \epsilon\}} \hspace{2em}\textrm{and}\hspace{2em} T^{\mdp}_{\textrm{mix}}(\epsilon) ~\defi~ \max_{i=1}^{n}{T^{\ecom_i}_{\textrm{mix}}(\epsilon)}.
	\]
 
 	The \emph{adjusted mixing time} of $\ecom$ and $\mdp$ are defined as their ergodic $\epsilon$-mixing time when $\epsilon = 1/4$, i.e. 
 	\[
 	\tmix^{\ecom}=\tmix^{\hat{\mchain}}~\defi~ T^{\hat{\mchain}}_{\textrm{mix}}(1/4) \hspace{2em}\textrm{and}\hspace{2em} T^{\mdp}_{\textrm{mix}}~\defi~ T^{\mdp}_{\textrm{mix}}(1/4).
 	\]
\end{definition}

For $\epsilon < 1/2$, we can obtain an upper bound of ergodic $\epsilon$-mixing time from the adjusted mixing time:

\begin{proposition}[{\cite[p.8]{Perla:2020}}]\label{prop:upper-mixing}
	Let $\mchain$  be an ergodic  chain and $\epsilon < 1/2$. Then $T_{\textrm{mix}}^{\mchain}(\epsilon) \leq \left\lceil \log_{2}{\frac{1}{\epsilon}} \right\rceil \tmix^{\mchain}$.
\end{proposition}

The following result states that we can compute the limit-average reward of the irreducible chain $\mchain$ from its ergodic transformation $\hat{\mchain}$:

\begin{proposition}[{\cite[\S8.5]{Puterman:1994}}]\label{prop:mxing-ergodic}
	Given an irreducible chain $\mchain$ and $M' = \alpha M + (1-\alpha)I$ is its ergodic transformation where $\alpha \in (0,1)$. Let $r$ and $\hat{r}$ be the limit-average reward of $\mchain$ and $\hat{\mchain}$ w.r.t. some reward function $\rfun$. Then $\hat{r} = \alpha \cdot r$.
\end{proposition}





\begin{lemma}\label{lm:sampling}
	Given an MDP $\mdp$  and $\epsilon,\delta > 0$. Let $\overline{\mdp}$ be the estimate of $\mdp$ by sampling every state-action pair $(s,a)$ in $\mdp$ at least  $N = \frac{1}{\delta'^2}\ln(\frac{2|A||S|^2}{\epsilon})$ times where $\delta' = \min{\{\delta,p^\mdp_{\textrm{min}}\}}$. Then:
	\[
	\Pr[\textrm{$\overline{\mdp} $ is an $(\mdp,\delta)$-estimate}] > 1 -\epsilon
	\]
\end{lemma}
\begin{proof}
	Let $e=(s,a,s')$ be a transition in $\mdp$ such that $p = P(s,a,s') > 0$. The sampling outcomes of $e$ are i.i.d. random variables $\{X_1,X_2,\ldots\}$ with the following Bernoulli distribution:
	\[
	\Pr[X_i = 1] ~=~ p \hspace{2em}\textrm{and}\hspace{2em} \Pr[X_i=0] ~=~ 1-  p
	\]
	
	Let $n \geq N$ and $S_n =\frac{\sum_{i=1}^{n} X_i}{n}$. Using Hoeffding's inequality, we deduce that:
	\[
	\Pr\left[|S_n - p| < \delta'\right] ~>~ 1- 2e^{-2n\delta'^2} ~\geq~  1- \frac{\epsilon}{|A||S|^2}
	\]
	
	Note that if $|S_n - p| < \delta'$ then  $|S_n - p| < p_{\textrm{min}}^{\mdp}$ and therefore $S_n > 0$. Since there are $|A|\cdot|S|^2$ transitions to sample, we can use Bernoulli's inequality to obtain the following lower bound:
	\[
	\Pr\left[\textrm{$\overline{\mdp}$ is $(\mdp,\delta')$-estimate}\right] ~>~ \left( 1- \frac{\epsilon}{|A||S|^2} \right)^{|A||S|^2} ~\geq~ 1 - \epsilon
	\]
	 Finally,  $\delta' \geq \delta$ implies that every  $(\mdp,\delta')$-estimate is also $(\mdp,\delta)$-estimate. Hence, we are done.
\end{proof}


\begin{lemma}\label{lm:exact-solution} \rm
	Let $\overline{\mdp}$ be $(\mdp,\delta)$-estimate and $\rfun$ a reward function. There exists an algorithm that returns a pair $(\overline{\pi}^*,\overline{\vfuns}^*)$ where $\overline{\pi}^*$ is optimal w.r.t. $(\overline{\mdp},\rfun)$ and $\overline{\vfuns}^*$ is its limit-average reward.
\end{lemma}
\begin{proof}
 By~\cref{prop:opt-avg-pol}, it suffices  to show that for each policy $\pi$, we can compute its limit-average reward $\vfun{\overline{\mdp}}{\rfun}(\pi)$. Let $ \mathsf{EC}(\mdp,\pi) = \{\ecom_1,\ldots,\ecom_n\}$. By~\cref{prop:avg-policy}, $\vfun{\overline{\mdp}}{\rfun}(\pi) = \sum_{i=1}^{n} x_i \cdot y_i$ where $x_i = \reachcom^\mdp_\pi(\ecom_i)$ and $y_i = \rewardcom^\mdp_\pi(\ecom_i,\rfun)$. Suppose $\ecom_i = (S_i,r_i)$. We show how to compute $x_i,y_i$ exactly:
 
\begin{enumerate}
	\item {\bf Compute $x_i$}. Let $x_i^j$ denote the probability that the state $s_j \in S$ reaches $\ecom_i$ and $\mathsf{Pre}(S_i)$ the set of states that can reach $S_i$ with non-zero probability. Note that $\mathsf{Pre}(S_i)$ can be computed efficiently using standard graph algorithms like Breadth First Search. Note that $x_i = x^0_i$ and $\{x_i^j\}_{j = 0}^{|S|-1}$ are the unique solution of the following system of $|S|$ linear equations:
	\begin{equation}\label{eqn:reach-system}
		\begin{cases}
		x^j_i = 0,&\textrm{if $s_j \not\in \mathsf{Pre}(S_i)$}
		\\
		x^j_i = 1,&\textrm{if $s_j \in S_i$}
		\\
		x^j_i = \sum_{s_k \in S \backslash S_i} \left(\overline{P}(s_j,\pi(s_j),s_k) \cdot x^k_i + \sum_{s_k \in S_i} \overline{P}(s_j,\pi(s_j),s_k)\right), &\textrm{otherwise.}	
	\end{cases}
	\end{equation}
	\item {\bf Compute $y_i$}. Assume $S_i = \{s_{i_1},\ldots s_{i_k}\}$. By~\cite[\S 8.2.3]{Puterman:1994}, it is sufficient to find the unique solution $\{w_j\}_{j=1}^{k} \cup \{y_i\}$ of the following system of $k+1$ linear equations:
	\begin{equation}\label{eqn:reward-system}
			\left\{ 
		\begin{array}{lcl}
			w_1 &=& 0 
			\\
			w_1 + y_i &=&  r_1 +\sum_{j=1}^{k} \overline{P}(s_{i_1},\pi(s_{i_1}),s_{i_j})\cdot w_j
			\\
			&\ldots&
			\\
			w_k + y_i &=& r_k + \sum_{j=1}^{k} \overline{P}(s_{i_k},\pi(s_{i_k}),s_{i_j}) \cdot w_j
		\end{array} 
		\right.
	\end{equation}
	where $r_t \defi \sum_{j=1}^{k}\overline{P}(s_{i_{t}},\pi(s_{i_t}),s_{i_{j}}) \cdot \rfun(s_{i_t},\pi(s_{i_t}),s_{i_j})$.
\end{enumerate}

As a result, $\vfun{\overline{\mdp}}{r}(\pi)$ can be computed exactly. Hence, we are done.
\end{proof}

Next, we show that the error of the optimal limit-average reward $|\vfuns^*(\overline{\mdp},\rfun) - \vfuns^*(\mdp,\rfun)|$ can be made arbitrary small by increasing the accuracy of the MDP estimation:

\begin{proposition}\label{prop:upper-bounds}
	Let $\pi$ be a policy of the MDP $\mdp$ with the reward function $\rfun$, and  $\epsilon,\delta > 0$. Then every $(\mdp,\delta)$-estimate $\overline{\mdp}$ is also  $(\overline{\mdp}_{\pi},\delta)$-estimate. Furthermore, for every  $\ecom_i \in \mathsf{EC}(\mdp,\pi)$:
	\begin{enumerate}
		\item If $\delta  = \frac{\epsilon\log{(1-p_{\min}^{|S|})}}{6|S|^2\log{(\epsilon/6)}}$ then
		$\left|\reachcom^{\overline{\mdp}}_{\pi}(\ecom_i) - \reachcom^{\mdp}_{\pi}(\ecom_i)\right| ~\leq~ \epsilon$.
		\item If $\epsilon < 2$ and $\delta \in O\left(\left(\frac{\epsilon^2}{24|S|\lceil \log_2{\left(\frac{4}{\epsilon}\right)} \rceil\tmix^\mdp}\right)^2\right)$ then $\left|\rewardcom^{\overline{\mdp}}_{\pi}(\ecom_i,\rfun) - \rewardcom^{\mdp}_{\pi}(\ecom_i,\rfun)\right| \leq \epsilon$.
	\end{enumerate}
\end{proposition}
\begin{proof}
	1)~By \cite[\bf Lemma 4]{Perez2024}, if  $\delta \leq \frac{\epsilon}{3|S|K}$ then $\left|\reachcom^{\overline{\mdp}}_{{\pi}}(\ecom_i) - \reachcom^{\mdp}_{\pi}(\ecom_i)\right| ~\leq~ \epsilon$ where $K$ is the $\epsilon/3$-recurrence time~(\cite[\bf Definition~1]{Perez2024}).  Using~\cite[\bf Lemma 1]{Perez2024}, we can obtain the upper bound of $K$, i.e. $K \leq 2|S| \frac{\log{(\epsilon/6)}}{\log{(1-p_{\min}^{|S|})}}$. Thus $\delta = \frac{\epsilon\log{(1-p_{\min}^{|S|})}}{6|S|^2\log{(\epsilon/6)}} $ yields the desired result.
		
	2)~ Let $\mchain_i$ be the transition matrix of the irreducible chain induced  $\ecom_i$. Consider its ergodic transformation $\hat{\ecom_i}$ induced by the transition matrix $\hat{\mchain_i} = 1/2(\mchain_i + I)$. Let $\rewardcom^{\mdp}_{\pi}(\ecom_i,\rfun,T)$ be the average reward of the first $T$-step in $\ecom$ (with a fixed initial state). By~\cite[\bf Simulation Lemma]{Kearns:2002},  if  $T$ is an upper bound of $T_{\epsilon/4}$ --- the $\epsilon/4$-return mixing time of $\hat{\ecom_i}$ (\cite[\bf Definition 5]{Kearns:2002}) --- and $\delta \in O\left(\left(\frac{\epsilon}{2|S|T}\right)^2\right) $ then $\left|\rewardcom^{\mdp}_{\pi}(\hat{\ecom_i},\rfun,T) - \rewardcom^{\overline{\mdp}}_{\pi}(\hat{\ecom_i},\rfun,T)\right| \leq \epsilon/2$. Using~\cite[\bf Lemma~1]{Kearns:2002} and~\cref{prop:upper-mixing}, we can obtain the upper bound $T$, i.e. $T_{\epsilon/4} \leq \frac{12\tmix^{\mdp}(\epsilon/4)}{\epsilon} \leq \frac{12\lceil \log_2{\left(\frac{4}{\epsilon}\right)} \rceil\tmix^\mdp}{\epsilon}$. Thus, if $\delta \in O\left(\left(\frac{\epsilon^2}{24|S|\lceil \log_2{\left(\frac{4}{\epsilon}\right)} \rceil\tmix^\mdp}\right)^2\right)$ then: 
		\[
		\left|\rewardcom^{\mdp}_{\pi}(\hat{\ecom_i},\rfun) - \rewardcom^{\overline{\mdp}}_{\pi}(\hat{\ecom_i},\rfun)\right| ~=~ \lim_{T \rightarrow \infty}{\left|\rewardcom^{\mdp}_{\pi}(\hat{\ecom_i},\rfun,T) - \rewardcom^{\overline{\mdp}}_{\pi}(\hat{\ecom_i},\rfun,T)\right|} ~\leq~ \epsilon/2
		\]

By~\cref{prop:mxing-ergodic}, $\left|\rewardcom^{\mdp}_{\pi}(\ecom_i,\rfun) - \rewardcom^{\overline{\mdp}}_{\pi}(\ecom_i,\rfun)\right| = 2\left|\rewardcom^{\mdp}_{\pi}(\hat{\ecom_i},\rfun) - \rewardcom^{\overline{\mdp}}_{\pi}(\hat{\ecom_i},\rfun)\right| \leq \epsilon$ as desired.
\end{proof}


\begin{lemma}\label{lm:close-optimal}
	Given an MDP $\mdp$, a reward function $\rfun$, a positive lower bound $\beta$ satisfying $0 < \beta \leq \min{\{p^\mdp_{\min},1/\tmix^\mdp\}}$. Then for every $\epsilon \in(0,2)$, we can compute some $\delta > 0$ from $\{|S|,\epsilon,\beta\}$ such that for every $(\mdp,\delta)$-estimate $\overline{\mdp}$, we have:
	\begin{enumerate}
		\item   $|\vfun{\overline{\mdp}}{\rfun}(\pi) - \vfun{\mdp}{\rfun}(\pi)| \leq \epsilon$ for every policy $\pi$.
		\item  $|\vfuns^*(\overline{\mdp},\rfun) - \vfuns^*(\mdp,\rfun)| \leq \epsilon$.
	\end{enumerate}
\end{lemma}
\begin{proof} Let $\mathsf{EC}(\mdp,\pi) = \{\mathcal{C}_1,\ldots,\mathcal{C}_n\}$. Due to disjointness, we deduce that $n \leq |S|$. Let $\epsilon' = \frac{\epsilon}{2|S|}$. For every $\ecom_i \in \mathsf{EC}(\mdp,\pi)$:
	\begin{enumerate}
		\item By~\cref{prop:upper-bounds}.1, we pick $\delta_1 =\frac{\epsilon'\log{(1-\beta^{|S|})}}{6|S|^2\log{(\epsilon'/6)}}$. Then every $(\mdp,\delta_1)$-estimate $\overline{\mdp}$ satisfies $\left|\reachcom^{\overline{\mdp}}_{\pi}(\ecom_i) - \reachcom^{\mdp}_{\pi}(\ecom_i)\right| \leq \epsilon'$. By~\cref{prop:upper-bounds}.2, if $ \delta_2 \in O\left(\left(\frac{\epsilon^2}{24|S|\lceil \log_2{\left(\frac{4}{\epsilon}\right)} \rceil\tmix^\mdp}\right)^2\right)$ then every $(\mdp,\delta_2)$-estimate $\overline{\mdp}$ satisfies $\left|\rewardcom^{\overline{\mdp}}_{\pi}(\ecom_i,\rfun) - \rewardcom^{\mdp}_{\pi}(\ecom_i,\rfun)\right| \leq \epsilon'$. Now, let $\delta = \min{\{\delta_1,\delta_2\}}$. Then every $(\mdp,\delta)$-estimate $\overline{\mdp}$ satisfies:
		\[
		\begin{array}{lll}
			\left|\vfun{\overline{\mdp}}{\rfun}(\pi) - \vfun{\mdp}{\rfun}(\pi)\right| &=& \left|\sum_{i=1}^{n}\left(\reachcom^{\overline{\mdp}}_{\pi}(\ecom_i)\cdot\rewardcom^{\overline{\mdp}}_{\pi}(\ecom_i,\rfun) - \reachcom^{\mdp}_{\pi}(\ecom_i)\cdot\rewardcom^{\mdp}_{\pi}(\ecom_i,\rfun)\right)\right|
			\\
			&\leq& \sum_{i=1}^{n} \reachcom^{\overline{\mdp}}_{\pi}(\ecom_i)\left|\rewardcom^{\overline{\mdp}}_{\pi}(\ecom_i,\rfun) - \rewardcom^{\mdp}_{\pi}(\ecom_i,\rfun)\right| 
			\\
			&&~+~\sum_{i=1}^{n}\rewardcom^{\mdp}_{\pi}(\ecom_i,\rfun)\left|\reachcom^{\overline{\mdp}}_{\pi}(\ecom_i) - \reachcom^{\mdp}_{\pi}(\ecom_i)\right| 
			\\
			&\leq& \sum_{i=1}^{n} 2\epsilon' ~\leq~ 2|S|\epsilon' ~=~ \epsilon.
		\end{array}
		\]
		\item 	Let $\delta$ be defined as in 1) and $\overline{\pi}^*$ the  $\rfun$-optimal policy. Then:
		\[
		\vfuns^*(\overline{\mdp},\rfun) ~=~ \vfun{\overline{\mdp}}{\rfun}(\overline{\pi^*}) ~\leq~ \vfun{\mdp}{\rfun}(\overline{\pi^*}) + \epsilon ~\leq~ \vfuns^*(\mdp,\rfun) + \epsilon
		\]
		
		Similarly, one can show that $\vfuns^*(\mdp,\rfun) \leq \vfuns^*(\overline{\mdp},\rfun) + \epsilon$. Hence, we are done.
	\end{enumerate}
\end{proof}




\begin{proof}[\bf Proof of~\cref{thm:learning-optimal}]
	Consider the product MDP $\mdp' = \mdp \ltimes \rfun$ with the induced reward function~$\rfun'$. Note that $p^{\mdp \ltimes \rfun}_{\min}=p^{\mdp}_{\min}$.  Our algorithm has the following steps:
	\begin{enumerate}
		\item Using~\cref{lm:close-optimal}, we can compute some $\delta' > 0$ from $\{|S \times U|,\delta,\beta'\}$ such that every $(\mdp',\delta')$-estimate $\overline{\mdp}$ satisfies $|\vfuns^*(\overline{\mdp},\rfun) - \vfuns^*(\mdp',\rfun)| \leq \delta$.
		\item Using~\cref{lm:sampling}, we sample each state-action pair $((s,u),a)$ in $\mdp'$ at least $N = \frac{1}{\delta''^2}\ln{(\frac{2|A||S\times U|^2}{\epsilon})}$ times where $\delta''=\min{\{p_{\min},\delta'\}}$ to obtain $\overline{\mdp}$ such that $\Pr\left[\textrm{$\overline{\mdp}$ is an $(\mdp',\delta')$-estimate}\right] > 1 - \epsilon$.
		\item Using~\cref{lm:exact-solution}, we compute the  optimal policy of $\overline{\mdp}$ and its optimal limit-average reward $(\overline{\pi}^*,\overline{\vfuns}^*)$. As a result, we can deduce that $\Pr[\vfun{\mdp'}{\rfun}(\overline{\pi}^*) ~\geq~ \vfuns^*(\mdp',\rfun) - \delta] > 1 -\epsilon$.
		\item We turn the deterministic memoryless $\overline{\pi}^*$ for $\mdp'$ into a deterministic finite-memory policy $\pi^*$ for $\mdp$ (i.e. by tracking the state of the reward machine $\rfun$) and output the policy $\pi^*$ as the final result. Note that such transformation does not change the limit-average reward of the policy, i.e.~$\vfun{\mdp}{\rfun}(\pi^*) = \vfun{\mdp'}{\rfun}(\overline{\pi}^*)$. Hence, $\Pr[\vfun{\mdp}{\rfun}(\pi^*) ~\geq~ \vfuns^*(\mdp,\rfun) - \delta] > 1 -\epsilon$.
	\end{enumerate}
\end{proof}


==> limit.tex <==
\lxb{Integrating Leon's part into the paper}

\textbf{Proposition 1} (\cite{Perez2024}). There is an algorithm $\omega$-PAC which inputs (1) a simulator for the labeled MDP $\mathcal{M}$, (2) an LTL formula $\varphi$, (3) $p > 0$, a lower bound on the positive transition probabilities in $\mathcal{M}$, (4) $\varepsilon, \delta > 0$, and outputs a policy $\pi$ such that $\Pr[\mathcal{J}_\varphi^{\mathcal{M}}(\pi) \geq \mathcal{J}^*(\mathcal{M}, \varphi) - \varepsilon] \geq 1 - \delta.$

\begin{wrapfigure}{L}{0.4\textwidth}
	\begin{minipage}{0.4\textwidth}
		\begin{algorithm}[H]
			\caption{RL for LTL in the limit}\label{alg:cap}
			\begin{algorithmic}
				\Require $\mathcal{M}, \varphi$
				\State $n \gets 0$
				\While{true}
				\State $\mathrel{n{+}{+}}~;~p,\varepsilon \gets 1/n~;~ \delta \gets 1/n^2$
				\State $\pi_n \gets \omega\text{-PAC}(\mathcal{M}, \varphi, p, \varepsilon, \delta)$
				\EndWhile
			\end{algorithmic}
		\end{algorithm}
	\end{minipage}
\end{wrapfigure}


We propose \cref{alg:cap}  that circumvents the requirement of knowing $p$ by iteratively guessing increasingly small values. Similar techniques has been employed for reinforcement learning with reward-based specifications \cite{Brafman:2003,Kearns:2002}. The algorithm proceeds in stages, beginning with stage $n = 1$.

\textbf{Theorem}. \cref{alg:cap} converges in the limit.

\begin{proof}
	By definition, we must show \[
	\Pr\left[\lim_{n \to \infty} \mathcal{J}_\varphi^{\mathcal{M}}(\pi_n) = \mathcal{J}^*(\mathcal{M}, \varphi)\right] = 1.
	\]
	It suffices to show that
	\[
	\mathbb{E}\left[\# \{n \mid \mathcal{J}_\varphi^\mathcal{M}(\pi_n) < \mathcal{J}^*(\mathcal{M}, \varphi) - 1/n \}\right] < \infty.
	\]
	Let $p_\text{min}$ be the smallest positive transition probability in $\mathcal{M}$. For stages $n \geq \lceil 1 / p_\text{min}  \rceil$, each call to the $\omega$-PAC subroutine is subject to the formal guarantee in Proposition 1. Consequently, we have
	\[
	\Pr[\mathcal{J}_\varphi^\mathcal{M}(\pi_n) < \mathcal{J}^*(\mathcal{M},\varphi) - 1/n] < \frac{1}{n^2}
	\]
	by choice of $\epsilon$ and $\delta$ in stage $n$. Linearity of expectation yields
	\begin{align*}
		&\mathbb{E}\left[\# \{n \geq \lceil 1 / p_\text{min} \rceil \mid \mathcal{J}_\varphi^\mathcal{M}(\pi_n) < \mathcal{J}^*(\mathcal{M}, \varphi) - 1/n \}\right] \\
		= &\sum_{n \geq \lceil 1 / p_\text{min} \rceil} \Pr[\mathcal{J}_\varphi^*(\pi_n) < \mathcal{J}^*(\mathcal{M},\varphi) - 1/n] \\
		\leq &\sum_{n \geq \lceil 1 / p_\text{min} \rceil} \frac{1}{n^2} \leq \sum_{n \geq 1} \frac{1}{n^2} = \frac{\pi^2}{6}.
	\end{align*}
	We conclude
	\begin{align*}
		&\mathbb{E}\left[\# \{n \mid \mathcal{J}_\varphi^\mathcal{M}(\pi_n) < \mathcal{J}^*(\mathcal{M}, \varphi) - 1/n \}\right] \\
		\leq \ &\lceil 1 / p_\text{min} \rceil + \mathbb{E}\left[\# \{n \geq \lceil 1/p_\text{min} \rceil \mid \mathcal{J}_\varphi^\mathcal{M}(\pi_n) < \mathcal{J}^*(\mathcal{M}, \varphi) - 1/n \}\right] \\
		\leq \  &\lceil 1 / p_\text{min} \rceil + \frac{\pi^2}{6} < \infty
	\end{align*}
	as needed.
\end{proof}

Note that the algorithm does not meet the precise definition of convergence in the limit since computing $\pi_n$ can require performing more than $n$ total actions in $\mathcal{M}$. This can be easily fixed by dilating the sequence of policies. Each time the $\omega$-PAC subroutine performs an action in $\mathcal{M}$, we simply output the most recently computed policy until the next policy is ready. Since stuttering preserves limits of convergent sequences, we obtain true convergence in the limit.

==> motivation.tex <==
Reinforcement learning algorithms aim to produce policies which achieve near-optimal scores with respect to a provided score-assigning specification. The most commonly used specifications are transition-based reward schemes. While reward-based specifications have been extensively studied, their low-level nature makes it difficult to capture natural objectives such as safety and reachability. Indeed, these infinite-horizon objectives are known to be inexpressible within the commonly used framework of discounted rewards \cite{Alur:2022, Yang2022}. Consequently, recent work has investigated the use of high-level logical formulas to score policies.

One popular choice of specification language is Linear Temporal Logic (LTL). Several reinforcement learning algorithms for LTL specifications have been proposed \cite{Perez2024, Brazdil:14, Voloshin:22, FuT:14, Shao:23}. Their formal guarantees vary, and each algorithm assumes some knowledge of the MDP's unknown structure (e.g. its transition probabilities). This knowledge requirement runs counter to the standard assumptionless framework of reinforcement learning, and raises the question as to which formal guarantees can be achieved without additional parameters.

Existing work provides only a partial answer: no assumptionless RL algorithm for LTL specifications can possess PAC guarantees \cite{Alur:2022}. However, until now, it has remained open whether more lax convergence guarantees are achievable. By way of a novel specification translation from LTL to average reward, we achieve an assumptionless convergence guarantee. At the same time, we situate the expressiveness of LTL specifications with respect to the well-studied class of average reward specifications.

==> related.tex <==
\section{Related Work}

{\bf LTL learning} 

{\bf Limit average rewards} Discount rewards can lead to sub-optimal policies if there are short-term payoffs that look more attractive. 

\begin{enumerate}
	\item Algorithms and tools for translating LTL to DRA:\cite{Klein:2006,Klein:2007,Babiak:2013}
	\item \cite{Wolff:12}: Find the policy that maximize the probability of satisfying the LTL constraint. Reduce to Stochastic shortest Path problem to reach AMECs.Assumptions: (1)known non-zero probability transitions in the MDP and (2) all stationary control policies are proper, i.e. there is a positive probability of reaching terminating states in at most $n$ steps, regardless of the initial states and transition matrices. Condition (2) is guaranteed after computing the product MDP. SO basically only need (1). Also contain good definition for EC. Compute the reachability prob directly instead of reducing to rewards.
	
	"The (worst-case) size of the deterministic Rabin automatonis doubly-exponential in the length of the LTL formula [8].Experimental work in [13] has shown that deterministic Rabinautomaton sizes are often exponential or lower for manycommon types of LTL formulae. Also, there are fragmentsof LTL, which include all safety and guarantee properties,that generate a determinstic Rabin automaton whose size is singly-exponential in the length of the formula [2]."
	
	\item \cite{Ding:14}:   Find the policy with the minimal average cost per cycle over all policies that maximize the probability of satisfying LTL. Use DRA and therefore AMECs. Assumption: the MDP is communicating and known transitions. e Dynamic Programming
	
	\item \cite{Voloshin:22}.  Find the policy that minimizes the combined cost (average-cost and transient cost). Use product MDP and LDBA. Compute the AMECs. Assumptions: lower bounds on probability, minimal cost is non-zero. Based on the lower bound, sample the MDP for the transitions. Attain PAC-approximation (with the assumption that the transition probability is constant).
	
	\item \cite{Bozkurt:2019}: Maximize prob of satisfying LTL. Assumption: known transitions. Use LDBA and Q-learning.
	\item \cite{Cai:2023}: Maximize prob of satisfying LTL. Assumption: known transitions. Use LDBA. Use Dynamic Programming.
	\item \cite{Hosein:2023} Maximize prob of satisfying LTL. Assumption: suitable discounted factor. Use LDBA and modified Q-learning. The LDBA is constructed on-the-fly.
	\item \cite{Sadigh:2014} Maximize prob of satisfying LTL. use Temporal Difference Learning (generalized Q-Learning/variant). Use DRA. Assumption: suitable discount factor and reward for rejecting states.
	\item \cite{FuT:14}: Maximize the probability of satisfying LTL. PAC-approximation. Use variant of R-max algorithm (average reward). Assumption: mixing time is known ("They defined the $\epsilon$-return mixing time ofa policy $\pi$ to be the smallest value of $T$ after which $\pi$ guarantees an expected payoff of at least $J(\pi)-\epsilon$")
\end{enumerate}

\lxb{
\begin{enumerate}
	\item Survey from \cite{Mahadevan:2004} is good for beginners but maybe outdated (1996). 
	\item \cite{Yang:2016}: A paper from Prof. Bo An's group. Also contain good summary about other average rewards papers. Model-free. "They (model-free algorithms) all use an adaptive shiftingvalue to approximate the optimal average reward to avoidthe unboundedness of Q-values. Their learning processes arehowever typically sensitive to input parameters and may often result in long execution time or even non-convergence." The authors claim that their approach can "overcome the instability and improve scalability of average reward RL". Assumptions: The MDP is irreducible, aperiodic, and ergodic; that is, under any stationary policy, the generatedMarkov chain is communicating and has a recurrent state.
	\item Model-free algorithms: R-learning~\cite{Schwartz:1993,Singh:1994}, SMART~\cite{Das:1999}, RVI Q-learning~\cite{Abounadi:2001,Li:2012}, GR-learning~\cite{Gosavi:2004}, and CSV-Learning~\cite{Yang:2016}.
	\item Model-based algorithms: Regret-model based. Copied from~\cite{Yang:2016}: "RM algorithms keep being optimistic about poorly understood states and actions (i.e., states and actions with high uncertainty) in order to encourage exploration. They estimate the MDP using some sampling techniques. Specifically, UCRL~\cite{Auer:2006} and UCRL2~\cite{Auer:2008} use two upper confidence (UC) values about the reward function and transition function; ineach episode a policy is generated based on the MDP modeland UCs (\cite{Auer:2006,Auer:2008}). PSRL~\cite{Ian:2013} uses posterior sampling: in each episode, it samples an MDP fromthe posterior distribution and then generates a policy."

	\item \cite{Schwartz:1993}: R-learning, the first learning algorithm for average rewards. Assume that all policies are unichain. Model-free. "This is a two-time-scale algorithm that carries
	out a value iteration-type step to update values of state-action pairs and updates concurrently an estimate of the optimal average cost using the immediate reward along
	with an adjustment factor. The idea is to obtain a good estimate for the average cost
	while searching for the optimal policy using a value iteration-type update."
	\item \cite{Singh:1994}: Also R-learning.
	\item \cite{Abounadi:2001} "RVI Q-learning uses the Q-values of a reference state as the shifting value". Model-free. Same assumptions as \cite{Yang:2016}.
\end{enumerate}
}





\dw{todo:
\begin{itemize}
    \item \url{https://arxiv.org/pdf/1909.07299.pdf}
    \item \url{https://arxiv.org/pdf/1810.00950.pdf}
    \item \url{https://arxiv.org/pdf/1909.05304.pdf}
    \item \url{https://papers.nips.cc/paper_files/paper/2023/file/95827e011b9e899f189a01fe2f4ef316-Paper-Conference.pdf}
    \item \url{https://arxiv.org/pdf/2210.05308.pdf}
    \item \url{https://www.roboticsproceedings.org/rss10/p39.pdf}
    \item \url{https://arxiv.org/pdf/1902.00778.pdf}
    \item ...
\end{itemize}
}
